Mechanics-based solution verification for porous media models

This paper presents a new approach to verify accuracy of computational simulations. We develop mathematical theorems which can serve as robust a posteriori error estimation techniques to identify numerical pollution, check the performance of adaptive meshes, and verify numerical solutions. We demonstrate performance of this methodology on problems from flow thorough porous media. However, one can extend it to other models. We construct mathematical properties such that the solutions to Darcy and Darcy-Brinkman equations satisfy them. The mathematical properties include the total minimum mechanical power, minimum dissipation theorem, reciprocal relation, and maximum principle for the vorticity. All the developed theorems have firm mechanical bases and are independent of numerical methods. So, these can be utilized for solution verification of finite element, finite volume, finite difference, lattice Boltzmann methods and so forth. In particular, we show that, for a given set of boundary conditions, Darcy velocity has the minimum total mechanical power of all the kinematically admissible vector fields. We also show that a similar result holds for Darcy-Brinkman velocity. We then show for a conservative body force, the Darcy and Darcy-Brinkman velocities have the minimum total dissipation among their respective kinematically admissible vector fields. Using numerical examples, we show that the minimum dissipation and total mechanical power theorems can be utilized to identify pollution errors in numerical solutions. The solutions to Darcy and Darcy-Brinkman equations are shown to satisfy a reciprocal relation, which has the potential to identify errors in the numerical implementation of boundary conditions.

==> Sections/S1_Brinkman_Introduction.tex <==
%************************************************;
%                                                ;
%  NAME                                          ;
%    S1_MBrinkman_Introduction.tex               ;
%                                                ;
%************************************************;
\section{INTRODUCTION}
\label{Sec:MDarcy_Introduction}
Porous media models are widely employed to make predictions 
in subsurface modeling which typically involves complex 
geometries and heterogeneous material properties. It 
therefore is necessary in subsurface modeling to 
rely on numerical simulations to solve realistic problems 
so as to make critical engineering decisions. For a problem 
with no known analytical or reference solution (which is 
typically the case in subsurface modeling), it becomes a 
non-trivial task for scientists to ensure that the employed 
numerical formulations and simulators are sufficiently 
accurate. Below are some specific challenges that a 
computational scientist may face in using numerical 
simulators:
\begin{enumerate}[(i)]
\item How much mesh refinement is required to obtain 
  solutions with desired degree of accuracy for a problem 
  that does not have an analytical or reference solution?
\item Will the chosen mesh be able to resolve 
  singularities in the solution and avoid 
  pollution errors? That is, 
  can we identify whether a particular type 
  of mesh suffers from pollution errors for 
  a problem with singularities?
\item Has the computer implementation been done properly?
\item Is the chosen numerical formulation accurate/appropriate 
  for the chosen problem?
\end{enumerate}
%
In the literature, one finds the usual approach of 
employing tools from functional analysis to obtain 
\emph{a priori} estimates and assess stability. For 
example, see \citep{Brezzi_Fortin,I_Babuska_FEM_2001}. 
%
On the other hand, this paper aims to address the 
aforementioned challenges 
for popular porous media models by providing various 
\emph{a posteriori} techniques with firm mechanics 
underpinning. It needs to be emphasized that the 
techniques presented in this paper will not be able 
to \emph{completely} address the aforementioned 
challenges. For example, there is currently no 
methodology that can judge with certainty the 
correctness of a computer implementation. The 
proposed techniques are no exception. However, 
the proposed \emph{a posteriori} techniques can 
be judiciously utilized to increase the confidence 
or detect shortcomings of a computer implementation 
and to assess the accuracy of numerical solutions. 

%===========================================;
%  Subsection: Popular porous media models  ;
%===========================================;
\subsection{Popular porous media models}
The simplest and yet the most popular model that subsurface 
modelers use is the Darcy model \citep{Darcy_1856}, which 
describes the flow of an incompressible fluid in a rigid 
porous media. The Darcy model has been employed in several 
branches of engineering and in several important technological 
applications. Some specific examples include groundwater 
hydrology \citep{Raats_Rational_Thermodynamics_1984, 
  Munaf_groundwater_v3_p231_1993_Math_Model_Meth_App_Sci}, 
enhanced oil recovery \citep{Minkoff_v38_p37_2003_J_Petr_Sci_Eng}, and 
simulation of flow of resin in composite manufacturing 
\citep{Nakshatrala_composite_mold_v27_p65_2006_Polymer_Composites,
  SH_Lee_resin_simul_v114_p1803_2009_J_App_Polymer_Sci}. The 
Darcy model has also been a cornerstone for the theoretical 
development of mixture theories \citep{Bowen,Boer_TPM}. However, 
the Darcy equations posed several challenges to the finite 
element community but played a crucial role in the 
development of mixed and stabilized formulations 
\citep{Brezzi_Fortin,Masoud_mixed_Darcy_v191_p4341_2002_CMAME,
Nakshatrala_mixed_Darcy_v195_p4036_2006_CMAME}. These equations 
have received considerable attention even from the mathematical 
community, especially in the area of mathematical homogenization 
\citep{Hornung}.
%
Brinkman \citep{Brinkman_ASR_1947_vA1_p27, Brinkman_ASR_1947_vA1_p81} 
proposed a popular extension to the Darcy model which is commonly 
referred to as the Darcy-Brinkman model. In addition to drag between 
the fluid and porous solid, Darcy-Brinkman model accounts for 
friction between fluid layers. 

The Darcy and Darcy-Brinkman models are adequate 
for most of the civil engineering and geotechnical 
applications in which the velocities and its gradient 
are small. It is, however, not possible 
to obtain analytical solutions under these models, and 
one commonly seeks numerical solutions for realistic 
problems. Some notable numerical formulations for Darcy 
and Darcy-Brinkman equations are 
\citep{Chavent_mixed_FEM_v47_p93_1984_CMAME, 
Ewing_mixed_FEM_Reservoir_v47_p161_1984_CMAME, 
Durlofsky_mixed_FVM_v30_p161_1994_Water_Resou_Reser, 
Arbogast_mixed_FEM_v34_p828_1997_SIAM_J_Nume_Anal, 
Masoud_mixed_Darcy_v191_p4341_2002_CMAME, 
Brezzi_mixed_Darcy_v22_p119_2005_SIAM_J_Sci_Compu, 
Nakshatrala_mixed_Darcy_v195_p4036_2006_CMAME, 
Burman_stabilized_Darcy_v198_p35_2007_J_Compu_App_Math, 
Nakshatrala_Rajagopal_IJNMF_2011_v67_p342, 
Nakshatrala_unsteady_Brinkman_v68_p642_2012_IJNMF}.
%
The question that still remains is how to verify 
the accuracy of numerical solutions, especially for 
realistic problems. This paper addresses this issue 
by providing several \emph{a posteriori} techniques to 
verify the accuracy of numerical solutions which 
falls under a current active area of research of 
validation and verification. 

%===============================================;
%  Subsection: Validation and verification V&V  ;
%===============================================;
\subsection{Validation and verification (V\&V)}
Errors can arise in both physical modeling and numerical 
simulation. The study of errors due to physical modeling 
is referred to as validation, and the study of error in a 
numerical simulation is referred to as verification. As 
Blottner \citep{Blottner_1990_v27_p113_122_J_spc_rock} 
nicely puts it, validation is to solve ``\emph{right 
governing equations}'' and verification is to solve  
``\emph{governing equation right}''.
%
Validation errors arise when a model is used out of 
its application range. Boundary conditions 
are also an important source of validation 
errors. The validation is beyond the scope of this 
study, and the reader can consult 
\citep{Roache_Verification_and_Validation} and the 
references therein. 
%

The errors in the verification can arise from three 
broad sources including numerical errors, round-off 
errors (due to the finite precision arithmetic), and 
programming mistakes 
\citep{WL_Oberkampf_VV_v57_p345_2004_Appl_mech_rev}.
%
Basically, the verification is to ensure that the 
code produces a solution to the model with some 
degree of accuracy, and the numerical solution 
is consistent. Verification itself can be 
divided into two categories: verification of 
code and verification of calculation 
\citep{Roache_Verification_and_Validation}. 
%
%=======================================;
%  Subsubsection: Verification of code  ;
%=======================================;
%\subsubsection{Verification of code}
Verification of code addresses the question of whether 
the numerical algorithms have been programmed and 
implemented correctly in the code. The two currently 
popular approaches to verify a code are the 
\emph{method of exact solutions} (MES) 
and the \emph{method of manufactured solutions} (MMS). 
%
%In the MES, one first seeks exact solutions 
%often with simplifications to the equations 
%and/or the boundary conditions. The numerical 
%results with corresponding inputs are then 
%compared to the exact solutions. 
%%
%In the MMS, an analytical solution is manufactured 
%\emph{a priori} and a source term is then calculated 
%that satisfies the governing equations. 
%Steinberg and Roache \citep{S_Steinberg_1985_v57_p251_284_JCP} 
%advocate the combined use of the MMS and 
%grid convergence for the verification of code. 
%%
%If the code passes a desired number of test problems 
%constructed by MES and/or MMS, then the 
%code is certified to be verified adequately. This by 
%no means implies that the code is completely bug free. 
%
More thorough discussions on MES and MMS can be 
found in \citep{Verification_computer_codes_Knupp_2003, 
CJ_Roy_IJNMF_v2004_p599,Roache_Verification_and_Validation}.

%==============================================;
%  Subsubsection: Verification of calculation  ;
%==============================================;
%\subsubsection{Verification of calculation}
Verification of calculation (which is also referred to 
as solution verification) estimates the overall 
magnitude (not just the order) of the numerical errors 
in a calculation, and the procedure invariably involves 
\emph{a posteriori} error estimation 
\citep{Code_Verification_by_MMS_SANDIA}. The numerical 
errors in the solution verification can arise from two 
different sources including discretization errors and 
solution errors. The discretization errors refer to all 
the errors caused by conversion of the governing equations 
(PDEs and boundary conditions) into discrete algebraic 
equations whereas the solution errors refer to the 
errors in approximate solution of the discrete equations. 
The numerical errors may arise from insufficient mesh 
resolution, improper selection of time-step, and 
incomplete iterative convergence. For more details on 
verification of calculation, see 
\citep{CJ_Roy_IJNMF_v2004_p599,Code_Verification_by_MMS_SANDIA,
PJ_Roache_quantifi_uncertainty_CFD_v29_p_123_1997_Annu_Rev_Fluid_Mech,
Roache_Verification_and_Validation,I_Babuska_VV_v193_p4057_2004_CMAME,
WL_Oberkampf_AIAA_v36_p687,WL_Oberkampf_VV_v57_p345_2004_Appl_mech_rev}.

%=======================================;
%  Subsection: A posteriori techniques  ;
%=======================================;
\subsection{\emph{A posteriori} techniques}
The aim of \emph{a posteriori} error estimation is to assess 
the accuracy of the numerical approximation in the terms of 
\emph{known} quantities such as geometrical properties 
of computational grid, the input data, and the numerical 
solution. \emph{A posteriori} error techniques monitor 
various forms of the error in the numerical solution such 
as velocity, stress, mean fluxes, and drag and lift coefficients 
\citep{Becker_error_estimation_v10_p1_2001_Acta_Numerica}. Such 
error estimation differ from \emph{a priori} error estimates in 
that the error controlling parameters depend on \emph{unknown} 
quantities. \emph{A priori} error estimation investigates the 
stability and convergence of a solver and can give rough 
information on the asymptotic behavior of errors in 
calculations when grid parameters are changed appropriately 
\citep{M_Ainsworth_Error_estimates_FEM_v142_p1_88_1997_CMAME}.

In the current study, we propose new mechanics-based 
criteria that can be used to verify the accuracy and 
convergence of numerical solutions to Darcy and 
Darcy Brinkman equations. The solution verification 
requires confirmation of grid convergence which is 
one of the most common and reliable error estimation 
methods 
\citep{PJ_Roache_quantifi_uncertainty_CFD_v29_p_123_1997_Annu_Rev_Fluid_Mech}. 
Similar to other grid convergence studies, we address only 
solution verification. Since the aim of this paper is 
\emph{a posteriori} error estimation, we assume that 
the code has already been verified for the Darcy 
and Darcy-Brinkman class of problems so that 
programming mistakes are not an issue. Likewise, we are not also 
concerned with validation. It means that the Darcy and 
Darcy-Brinkman models are physically adequate to model 
the problems.

%=========================================;
%  Subsection: Organization of the paper  ;
%=========================================;
\subsection{Organization of the paper}
Section \ref{Sec:S2_Brinkman_GE} presents 
the governing equations arising from the 
Darcy and Darcy-Brinkman models. In Section 
\ref{Sec:S3_Brinkman_Theorems}, we propose 
various mathematical properties that the 
solutions to these governing equations 
satisfy. We also discuss how these 
properties can be utilized as robust 
\emph{a posteriori} criteria to assess 
the accuracy of numerical solutions.
%
Section \ref{Sec:S4_Brinkman_NR} presents several  
steady-state numerical results to illustrate the 
predictive capabilities of the proposed \emph{a 
  posteriori} criteria with respect to singularities, 
pollution errors, and discretization errors in the 
implementation of (Neumann) boundary conditions.
%
In Section \ref{Sec:S5_Brinkman_Marmousi}, 
we utilize synthetic reservoir data to 
demonstrate the usefulness of the proposed 
\emph{a posteriori} techniques, especially 
for problems involving spatially heterogeneous 
permeability properties.  
%
Section \ref{Sec:S6_Brinkman_Transient} discusses 
\emph{a posteriori} criteria for transient problems, 
and presents representative numerical results in 
support of the theoretical predictions. 
%
Finally, conclusions are drawn in Section 
\ref{Sec:S8_Brinkman_Closure}.  


